ITect: Scalable Information Theoretic Similarity for Malware Detection

Malware creators have been getting their way for too long now. String-based similarity measures can leverage ground truth in a scalable way and can operate at a level of abstraction that is difficult to combat from the code level. We introduce ITect, a scalable approach to malware similarity detection based on information theory. ITect targets file entropy patterns in different ways to achieve 100% precision with 90% accuracy but it could target 100% recall instead. It outperforms VirusTotal for precision and accuracy on combined Kaggle and VirusShare malware.

==> notes.tex <==
The results from Table 5 are not as good as the authors
suggest. For instance, on the packed_2 dataset the tool obtain 69\% detection with 5\% false positive. Why? The paper does not provide any answer. However, the authors tried to understand why results were good for the meta category and found out that the two families in that group contained in fact encrypted or compressed data (so, it basically worked by luck).

The benign-ware used in the experiments is packed, due to exe files have been used. 

60 test files are packed.
Borland 14
NET 31
PECompac 8
UPX 7
60/600

When the cutoff is less conservative, i.e., a 5\% of FP, this files are classified as malware, these files are misclassified. 



